LawSum: A weakly supervised approach for Indian Legal Document Summarization

Unlike the courts in western countries, public records of Indian judiciary are completely unstructured and noisy. No large scale publicly available annotated datasets of Indian legal documents exist till date. This limits the scope for legal analytics research. In this work, we propose a new dataset consisting of over 10,000 judgements delivered by the supreme court of India and their corresponding hand written summaries. The proposed dataset is pre-processed by normalising common legal abbreviations, handling spelling variations in named entities, handling bad punctuations and accurate sentence tokenization. Each sentence is tagged with their rhetorical roles. We also annotate each judgement with several attributes like date, names of the plaintiffs, defendants and the people representing them, judges who delivered the judgement, acts/statutes that are cited and the most common citations used to refer the judgement. Further, we propose an automatic labelling technique for identifying sentences which have summary worthy information. We demonstrate that this auto labeled data can be used effectively to train a weakly supervised sentence extractor with high accuracy. Some possible applications of this dataset besides legal document summarization can be in retrieval, citation analysis and prediction of decisions by a particular judge.

==> sections/Eg_Headnote.tex <==
\section{Headnote}

HEADNOTE: \\
     The respondent's  suit for	 the recovery  of money from
the  first  appellant's	 husband  was  decreed	and  in	 the
execution of  the decree  certain property  of the appellant
was  brought  to  sale.	 The  decree-holder  purchased	that
property.  The	 appellant's  husband  having  died  in	 the
meanwhile his  legal representatives  filed  an	 application
under order XXI, Rule 90 of the C.P.C. for setting aside the
sale. That application was dismissed by the executing court.
On the	appellant's appeal,  the sale  was set aside. At the
stage of  second appeal	 filed by the respondent the partiesH
entered into  a compromise with the leave of the court which
after  granting	  leave	 made  an  order  in  terms  of	 the
compromise. Under  a term  of the compromise, the appellants
agreed to  deposit, and	 the respondent	 agreed to receive a
sum of	Rs. 60,000/-  in full  and final  settlement of	 the
decree. It  was also stated that if the deposit was not made
on or  before the  stipulated date,  the sale  was to  stand
confirmed and  the second  appeal of  the respondent  was to
stand. Having  found it	 difficult to  deposit the  money in
terms of the compromise, the appellants filed an application
under Ss.  148 and  151 of  the C.P.C. praying that the time
for depositing	the money  in terms  of	 the  compromise  be
extended. The  High Court  dismissed this application on the
ground that  the Court	could not extend time where time had
been stipulated	 by the parties in the compromise arrived at
between them. \\
     In appeal	to this	 Court it was contended on behalf of
the appellants	that where  a compromise  had been  made the
order of  the Court,  it was open to the Court to extend the
time under s. 148 C.P.C. \\
     Allowing the  appeal and remanding the case to the High
Court to  dispose of  the execution  second appeal afresh in
accordance with the law. \\
    HELD: As  there was  no statutory compulsion to dismiss
the application	 under order  XXI, Rule	 90, C.P.C,  in	 the
absence of an agreement between the parties, the Court would
have decided the appeal arising out of tho application
468 \\
on the	merits. The  parties in	 the  instant  case  however
entered into  a compromise  and invited the court to make an
order in  terms of  the compromise, which the Court did. The
time for  deposit stipulated  by the parties became the time
allowed	 by   the  Court   and	this   gave  the  Court	 the
jurisdiction to extend time in appropriate cases. Time would
not be	extended ordinarily,  nor for  the mere	 asking	 but
would  be   granted  in	  rare	cases  to  prevent  manifest
injustice. Where  the contract	of the parties has merged in
the order of the Court the Court's freedom to act to further
the ends  of justice  would not	 stand curtailed.  The	High
Court was  in error  in thinking  that they  had no power to
extend time. \\
Hukumchand v.  Bansilal and  ors., A.I.R.	1968 SC	 86, held inapplicable.

==> sections/Eg_Info.tex <==
\section{Info}

Smt. Periyakkal $\&$ Others vs Smt. Dakshyani on 2 March, 1983 \\
Equivalent citations: 1983 AIR 428, 1983 SCR (2) 467 \\
Author: O C Reddy \\
Bench: Reddy, O. Chinnappa (J) \\
\\
PETITIONER: \\
SMT. PERIYAKKAL $\&$ OTHERS \\
\\
	Vs. \\
\\
RESPONDENT: \\
SMT. DAKSHYANI \\
\\
DATE OF JUDGMENT02/03/1983 \\
\\
BENCH: \\
REDDY, O. CHINNAPPA (J) \\
BENCH: \\
REDDY, O. CHINNAPPA (J) \\
PATHAK, R.S. \\
\\
CITATION: \\
 1983 AIR  428		  1983 SCR  (2) 467 \\
 1983 SCC  (2) 127	  1983 SCALE  (1)213 \\
 CITATOR INFO : \\
 D	    1988 SC 981	 (6,8) \\
\\
ACT: \\
Code of  Civil Procedure - order XXI, Rule 90-Scope of-
Parties entcred	 into a	 compromise with leave of Court that
appellants should  pay in Court before the stipulated date a
sum of	money in  full and  final setllement  of the decree-
Appellants  failed   to	 deposit   the	money  in  terms  of
compromise-Made an  application for  extension of  time-High
Court, if competent to extend time.

==> sections/Eg_Judgement.tex <==
\section{Judgement}
JUDGMENT: \\
CIVIL APPELLATE JURISDICTION: Civil Appeal No. 3527 of 1979. \\

Appeal by Special leave from the Judgment and order dated the 15th JaNuary, 1979 of the Karnataka High Court in Executive Second Appeal No. 89 of 1974.

Dr. Y.S. Chifale, R. B. Datar and Miss Madhu Mool Chandani for the Appellants.

S. C. Javali, Ranjit KtJmar and B. P. Singh for the Respondent.

The Judgment of the Court was delivered by CHINNAPPA REDDY, J. The respondent Dakshyani sued to recover a sum of RS. 7,324.86 paise from Narayana Swami, husband of the first appellant and father of the rest of the appellants. The suit was decreed with costs and, in execution of the decree, certain property situated in Bangalore City was brought to sale. The decree-holder purchased the property at the execution sale held on August 19, 1969, for a sum of Rs. 28,000. Narayana Swami having died in the meanwhile, his legal representatives, the present appellants, filed an application under the provisions of order 21 Rule 90 for setting aside the sale on various grounds. The Executing Court dismissed the application on March 28, 1973 but on an appeal preferred by the appellants the sale was set aside on July 31, 1974. The respondent filed a second appeal to the High Court of Karnataka. At the hearing of the second appeal the parties entered into a compromise with the leave of the Court, such leave being necessary since mally of the present appellants were minors then and are minors even now. The Court granted leave and made an order in terms of the compromise. The term of the compromise which we are concerned is that the present appellants agreed to deposit and the present respondent agreed to receive a sum of Rs. 60,000/-in full and final settlement of the decree. If the deposit was made on or before November 30, 1976, the sale which though confirmed by the Trial Court but set aside by the Appellate Court was to stand set aside and the second appeal of the respondent was to stand dismissed. If the amount of Rs. 60,000/- was not deposited on or before November 30, 1976 the second appeal was to stand allowed and the sale was to stand confirmed. Time was stated to be the essence of the contract between the parties. The applellants were permitted under the compromise, to raise funds by sale, mortgage etc. Of the property in question. The appellants failed to deposit the amount in terms of the compromise. It appeaIs that they were unable to raise the necessary funds as they could not evict the tenant who was in occupation of the property. Finally the appellants filed an application purporting to be under ss. 148 and 151 of the Civil Procedure Code to extend the time for depositing the sum of Rs. 60,000 in terms of the compromise dated June 24, 1976. The High Court dismissed the application on the ground that the Court could not extend time where time had been stipulated by the parties themselves in the compromise arrived at between them. The High Court purported to rely upon the decision of this Court in Hukumchand v. Bansilal and Ors.(l) Shri R. B. Datar Learned Counsel for the appellants urged that there was no limitation on the power of the Court to extend time under s. 148, c. P. c. and that where a compromise had been made an order of the Court, it was certainly open to the Court to extend time under s. 148 c. P. c. He relied upon the decision of the High Courts of Bombay and Calcutta in Marketing and Advertising Associates Pvt. Ltd. v. Telerad Pvt. Ltd.(2) Jadabendra Nath Mishra v. Manorama Debya(3). He distinguished the decision of this Court in Hukum Chand v. Bansilal. Shri Javali Learned Counsel for the respondent, on the other hand urged that time should not be extended by the Court, in law and on principle, where the parties themselves had agreed upon the time within which the amount was to be deposited.

In Hukamchand v. Bansilal the real question which was considered was, if a mortgaged property was sold in execution of a mortgage decree and if the application to set aside the sale under order 21 Rule 90 was dismissed but time was granted by consent of parties for depositing the decretal amount etc. could time be extended for depositing the decretal amount etc. to avert the confirmation of sale under order 34 Rule S, except with the consent of the parties. The answer was 'no'. .The Court said on the dismissal of an application under order 21 Rule 90, confir- mation of sale under order 21 Rule 92 had to follow as a matter of course. Order 34 Rule S merely permitted the deposit to be made at any time before confirmation of the sale and there could be no question of extending the time for such deposit. If parties agreed to have the con- firmation of sale postponed, further postponement would be possible by agreement of parties only. The Court would have no say in the matter. Sec. 148 C. P. C. would have no application. The position was clarified by the Court thus :

"The judgment-debtor mortgagor had the right to de- posit the amount at any time before confirmation of sale within 30 days after the sale or even more than 30 days after the sale under order XXXIV, Rule (S) (l) so long as the sale was not confirmed. If the amount had been deposited before the confirmation of sale, the judgment- debtors had the right to ask for an order in terms of order XXXlV, Rule 5 (1) in their favour. In this case an application under order XXI Rule 90 had been made and, therefore, the sale could not be confirmed immediately after 30 days which would be the normal course; the confirmation had to await the disposal of the application under order XXl, Rule 90. That application was disposed of on October 7, 1958 and was dismissed. It is obvious from the order sheet of October 7, 1958 that an oral compromise was arrived at between the parties in court on that day. By that compromise time was granted to the respondents to deposit the entire amount due to the decree-holder and the auction-purchaser by November 21, 1958. Obviously, the basis of the compromise was A that respondents withdrew their application, under order XXI, Rule 90 while the decree-holder society and the auction-purchaser appellant agreed that time might be given to deposit the amount upto November, 21,1958. If this agreement had not been arrived at and if the application under order XXI, Rule 90 had been dismis- sed (for example, on merits) on October 7, 1958, the court was bound under order XXI, Rule 92 (1) to confirm the sale at once. But because of the compromise between the parties by which the respondents were given time upto November 21, 1958 the court rightly postponed the question of confirmation of sale till that date by consent of parties. But the fact remains that the application under order XXI, Rule 90 had been dismissed on October 7, 1958 and thereafter, the court was bound to confirm the sale but for the compromise between the parties giving time upto November 21, 1958".
The Court then referred to the refusal of the Court to extend time by a fortnight on November 22, 1958 and further observed :-

"The executing court refused that holding that time upto Nov. 21, 1958 had been granted by consent and it was no longer open to it to extend that time. The executing court has not referred to order XXI, Rule 92 in its order, but it is obvious that the executing court held that it could not grant time in the absence of an agreement between the parties because order XX[, Rule 92 required that as the application under order XXI, Rule 90 had been dismissed the sale must be confirmed. We are of the view that in the circumstances it was not open to the executing court to extend time without consent of parties, for time between October 7, 1958 to November 21, 1958 was granted by consent of parties. Section 148 of the Code of Civil Procedure would not apply in these circumstances, and the executing court was right in holding that it could not extend time. Thereafter, it rightly confirmed the sale as required under order XXI, Rule 92 there being no question of the appli-

cation of order XXXIV, Rule S for the money had not been deposited on November 22, 1958 before the order J of confirmation was passed. Tn this view of the matter, we are of opinion that the order of the executing court refusing grant of time and confirming the sale was correct".
In the case before us, the situation Is totally different. Unlike the case of Hukam Chand v. Bansilal where there was a statuory compulsion to confirm the sale on the dismissal OF the application under order XXI Rule 90 and, therefore, postponement and further postponement of the confirmation of the sale could only be by the consent of the parties in the case before us, there was no statutory compulsion to dismiss the application under order XXI, Rule 90 in the absence of an agreement between the parties. The court would have then decided the appeal arising out of the application on the merits. The parties, however, entered into a compromise and invited the court to make an order in terms of the compromise, which the court did. The time for deposit stipulated by the parties became the time allowed by the court and this gave the court the jurisdiction to extend time in appropriate cases. Of course, time would not be extended ordinarily, nor for the mere asking. It would be granted in rare cases to prevent manifest injustice. True the court would not rewrite a contract between the parties but the court would relieve against a forfeiture clause; And, where the contract of the parties has merged in the order of the court, the court's freedom to act to further the ends of justice would surely not stand curtailed. Nothing said in Hukamchand's case militates against this view. We are, therefore, of the view that the High Court was in error in; thinking that they had no power to extend time. Even so, Shri Jawali submitted that this was not an appopriate case for granting any extension of time. We desire to express no opinion on that question. The High Court will decide that question. We accordingly, set aside that judgment dated 15th January, 1979, of the High Court and direct the High Court to dispose of I. A. No. VIII in Execution Second Appeal No. 89/74 in accordance with law. The parties will bear their own costs.

P.B.R.					     Appeal allowed.

==> sections/TODO.tex <==
% TODO:

% Questions
% 2. Analysis for Rhetorical Roles Identification : Compare with Dataset in the https://github.com/Law-AI/semantic-segmentation/blob/master/data/text/1953_L_1.txt with our techniue of preprocessing and rhetorical identification.
% 3. Confusion matrix for attorneys.
% 4. Add confusion matrix for different thresholds, should add for all for comparision
% 5. Examples are too big
% 6. Addition of Images and Charts. (As commented in the respective tex files)
% 7. Compare length of sentences in different nlp baselines datasets.
% 8. Results for Transformer Model


